Herd: Using multiple, smaller LLMs to match the performances of proprietary, large LLMs via an intelligent composer

Currently, over a thousand LLMs exist that are multi-purpose and are capable of performing real world tasks, including Q&A, text summarization, content generation, etc. However, accessibility, scale and reliability of free models prevents them from being widely deployed in everyday use cases. To address the first two issues of access and scale, organisations such as HuggingFace have created model repositories where users have uploaded model weights and quantized versions of models trained using different paradigms, as well as model cards describing their training process. While some models report performance on commonly used benchmarks, not all do, and interpreting the real world impact of trading off performance on a benchmark for model deployment cost, is unclear. Here, we show that a herd of open source models can match or exceed the performance of proprietary models via an intelligent router. We show that a Herd of open source models is able to match the accuracy of ChatGPT, despite being composed of models that are effectively 2.5x smaller. We show that in cases where GPT is not able to answer the query, Herd is able to identify a model that can, at least 40% of the time.

==> active_blackboard.tex <==
\subsection*{Active Blackboard}
The thalamus plays part of an active blackboard, and exhibits two way connection to the cortex. The thalamus processes the signals from the cortex, and extracts higher level meaning from the data, which it sends back to the cortex. We take advantage of this divorcing of data and compute, where one system holds the data and another processes it into higher level features. 

In Large language models, we find that an LLM is forced to both know a lot of data as well as be able to respond to queries in an intelligent way. This causes LLMs to be extremely large and datasets to be extremetly expensive to train on. To circumvent this, RAG [cite] and other efforts have attemped to feed data to LLMs. In this work, we also feed LLMs some input in context, from another open source LLM, chosen by a router. 

